TA-Dash: An Interactive Dashboard for Spatial-Temporal Traffic Analytics -- Demo Paper

In recent years, a large number of research efforts aimed at the development of machine learning models to predict complex spatial-temporal mobility patterns and their impact on road traffic and infrastructure. However, the utility of these models is often diminished due to the lack of accessible user interfaces to view and analyse prediction results. In this paper, we present the Traffic Analytics Dashboard ( TA-Dash), an interactive dashboard that enables the visualisation of complex spatial-temporal urban traffic patterns. We demonstrate the utility of TA-Dash at the example of two recently proposed spatial-temporal models for urban traffic and urban road infrastructure analysis. In particular, the use cases include the analysis, prediction and visualisation of the impact of planned special events on urban road traffic as well as the analysis and visualisation of structural dependencies within urban road networks. The lightweight TA-Dash dashboard aims to address non-expert users involved in urban traffic management and mobility service planning. The TA-Dash builds on a flexible layer-based architecture that is easily adaptable to the visualisation of new models.

==> 5_relatedwork.tex <==
%\section{Related Work}
%\label{sec:related}

%Visual analytics has been utilised in the mobility and transportation domain for a variety of purposed, including exploratory analysis of movement data as well as more advanced tasks of traffic modelling, forecasting, and planning \cite{Andrienko17}.
%The applications in this area range from complex GIS systems for historical data analytics to highly specialised visualisations of traffic flow for particular use cases.
%
%In contrast, the \dashboard provides a lightweight approach to explore and jointly analyse spatial-temporal patterns resulting from traffic analytic models visually on a layered map.   


%Recently, efforts has been made to make it easier for non-expert users to create data analytics workflows in the context of mobility analytics \cite{GottschalkTKIFD19}. The \dashboard dashboard facilitates lightweight visual analytics on top of heterogeneous urban information sources discussed in \cite{TempelmeierRLKM19}.
